Optimisation of the SVOM satellite strategy for the rapid follow-up of gravitational wave events

The SVOM satellite, to be launched in early 2024, is primarily devoted to the multi-wavelength observation of gamma-ray bursts and other higher-energy transients. Thanks to its onboard Microchannel X-ray Telescope and Visible-band Telescope, it is also very well adapted to the electromagnetic follow-up of gravitational wave events. We discuss the SVOM rapid follow-up strategy for gravitational wave trigger candidates provided by LIGO-Virgo-KAGRA. In particular, we make use of recent developments of galaxy catalogs adapted to the horizon of gravitational wave detectors to optimise the chance of counterpart discovery. We also take into account constraints specific to the SVOM platform. Finally, we implement the production of the SVOM observation plan following a gravitational wave alert and quantify the efficiency of several optimisations introduced in this work.

==> plots_cumus.tex <==
%\onecolumn

\begin{figure}
\begin{center}
\centering
\vspace{-15cm}
\includegraphics[width=0.8\columnwidth]{plots/cumulativ_plots/GW170817_grade.png}
\end{center}
\caption{Figures \ref{fig:GW170817_grade} to \ref{fig:grade_s190901ap}, cumulative observed grade of the SVOM-MXT simulation for GW170817, MS191222t and S190901ap (see section \ref{section:Tillingvsgaltar}).}
\label{fig:GW170817_grade}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}
\begin{center}
\centering
\includegraphics[width=0.8\columnwidth]{plots/cumulativ_plots/MS191222t_grade.png}
\end{center}
\caption{}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}
\begin{center}
\centering
\includegraphics[width=0.8\columnwidth]{plots/cumulativ_plots/S190901ap_grade.png}
\end{center}
\caption{}
\label{fig:grade_s190901ap}
\end{figure}


==> table_def_grades.tex <==
\begin{table}
  \hspace{0.5cm}
  \caption{\corr{Description of the naming convention used throughout this work.} \corr{We consider an observation plan with $N_{\mathrm{tiles}}$ tiles.
  The index $i$ runs over tiles and the index $j$ over  galaxies contained in a given tile and compatible with the considered 3D-skymap.
  The grade of each compatible galaxy is written $G_{\mathrm{gal,}j}$ (see text). }}
  \label{tab:naming}
  \begin{tabular}{ c c c}
    \hline
    Naming & Description  & Expression\\
    \hline
    Number of \lang{galaxies} of a tile & Number of compatible galaxies contained by tile $i$ & $N_{\mathrm{gal,} i}$\\
    %\hline
    Grade of a tile & Sum of the \lang{grades} of the compatible galaxies contained by the tile $i$ & $\sum_{j = 0}^{N_{\mathrm{gal,}i}} G_{\mathrm{gal,}j}$ \\
    \hline
    Number of observed \lang{galaxies} & Sum of the number of \lang{galaxies} of \lang{all} the tiles of the observation plan & $\sum_{i = 0}^{N_{\mathrm{tiles}}} N_{\mathrm{gal},i}$\\
    %\hline
    \corr{Observed grade}
    %Number of observed grade 
    & Sum of the \lang{grades} of \lang{all} the tiles of the observation plan & $\sum_{i = 0}^{N_{\mathrm{tiles}}} \sum_{j = 0}^{N_{\mathrm{gal},i}} G_{\mathrm{gal},j}$\\
    \hline
    Maximum of observed galaxy & Number of observed galaxy after the maximum number of tile computed by the observation plan & $\sum_{i = 0}^{N_{tile \, max}} N_{gal,i}$ \\
    %\hline
    Maximum of observed grade  & Number of observed grade after the maximum number of tile computed by the observation plan & $\sum_{i = 0}^{N_{tile \, max}} \sum_{j = 0}^{N_{gal,i}} G_{gal,j}$ \\
    \hline
  \end{tabular}

  \old{*** deux dernières lignes à corriger ***}
\end{table}




==> table_skymap.tex <==


